All Verdicts are Not Equal: Rethinking LLM Judge Reliability

LLM-as-a-Judge is the standard paradigm for NLP evaluation, yet its systemic reliability remains poorly understood despite being widely treated as a deterministic ground truth. We present a comprehensive reliability audit, stresstesting six frontier models across four benchmarks, five prompt formats, two presentation orders, three sampling temperatures, and ten repetitions per condition. Our empirical analysis reveals severe vulnerabilities: verdicts change across identical replications at temperature zero, position-order swaps flip the majority of verdicts on challenging tasks, and the most deterministic judge achieves perfect consistency by trivially repeating incorrect verdicts, agreeing with ground truth only 51% of the time. To formalize these multi-faceted failure modes, we introduce the trustworthy verdict rate (T ), a unified metric capturing the joint probability that an evaluation is reproducible, order-invariant, and accurate. UsingT , we derive a theoretical upper bound on accuracy imposed by position bias and show that reliability is item-specific rather than modellevel. Finally, we demonstrate that shifting from pairwise win-rate to holistic rubric scoring improves trustworthiness more than any single-format prompting intervention, offering an actionable framework for robust NLP evaluation.

==> empirical_vs_closed.tex <==
\section{Closed-Form vs.\ Empirical Trustworthy Rate}                                               
  \label{app:t_validation}               
   
  The closed-form decomposition $T = C \times (A - \varphi/2)$                                        
  (Eq~\ref{eq:trustworthy}) relies on two independence assumptions:                           
  \begin{itemize}
    \item[\textbf{A1.}] $\Pr(P{=}1 \mid N{=}1) = \Pr(P{=}1)$ ---
      order-invariance is independent of within-order reproducibility.                                
    \item[\textbf{A2.}] $\Pr(R{=}1 \mid N{=}1, P{=}1) = A_{\mathrm{dec}}$ ---                         
      among decisive pairs, accuracy equals the population decisive accuracy.                         
  \end{itemize}                                                                                       

  \noindent                                                                                           
  We validate these by comparing $T_{\mathrm{closed}} = C(A - \varphi/2)$                             
  against the directly computed joint probability                                                     
  $T_{\mathrm{emp}} = \Pr(N{=}1 \wedge P{=}1 \wedge R{=}1)$                                           
  for all 24 judge--dataset combinations at $T_{\mathrm{temp}}{=}0$.                                  
  For each evaluation cell $(p, j, f)$:                                                               
  $N{=}1$ iff the majority verdict is identical across all 10 repetitions                             
  in \emph{both} orders;                                                                              
  $P{=}1$ iff the canonical majority verdicts in AB and BA agree;                                     
  $R{=}1$ iff the overall majority verdict matches the ground-truth label.                            
  Table~\ref{tab:t_validation} reports both estimates and the per-assumption                          
  gaps.                                                                                               
                                                                                                      
  \begin{table*}[h!]                                                                                   
  \centering                                                                                          
  \small                                                                                              
  \caption{Closed-form $T_{\mathrm{closed}} = C(A - \varphi/2)$ vs.\                                  
  empirical $T_{\mathrm{emp}} = \Pr(N{=}1 \wedge P{=}1 \wedge R{=}1)$                                 
  across all 24 judge--dataset combinations at $T_{\mathrm{temp}}{=}0$.                               
  \textbf{A1 gap}: $\Pr(P{=}1 \mid N{=}1) - \Pr(P{=}1)$; positive means                               
  deterministic verdicts are \emph{more} order-invariant than average.                                
  \textbf{A2 gap}: $\Pr(R{=}1 \mid N{=}1, P{=}1) - A_{\mathrm{dec}}$;                                 
  positive means the deterministic-and-decisive subset is \emph{more}                                 
  accurate than the theoretical $A_{\mathrm{dec}}$.                                                   
  Both assumptions err conservatively in 20--21 of 24 cases, making                                   
  $T_{\mathrm{closed}}$ a lower bound on true trustworthiness.}                                       
  \label{tab:t_validation}                                                                            
  \begin{tabular}{ll rr r rr}                                                                         
  \toprule                                                                                            
  \textbf{Dataset} & \textbf{Judge}                         
    & $T_{\mathrm{closed}}$ & $T_{\mathrm{emp}}$                                                      
    & \textbf{Gap}                                          
    & \textbf{A1 gap} & \textbf{A2 gap} \\                                                            
  \midrule                                                  
  MT-Bench                                                                                            
    & Claude-Sonnet-4.6   & 0.583 & 0.627 & $+$0.044 & $+$0.020 & $+$0.037 \\                         
    & GPT-5.2             & 0.491 & 0.555 & $+$0.064 & $+$0.026 & $+$0.067 \\                         
    & Gemini-2.5-Pro      & 0.436 & 0.530 & $+$0.094 & $+$0.062 & $+$0.087 \\                         
    & GPT-4o              & 0.514 & 0.563 & $+$0.050 & $+$0.022 & $+$0.046 \\                         
    & Gemini-2.0-Flash    & 0.455 & 0.521 & $+$0.066 & $+$0.004 & $+$0.089 \\                         
    & Llama-3.3-70B       & 0.540 & 0.580 & $+$0.039 & $-$0.001 & $+$0.047 \\                         
  \cmidrule(l){1-7}                                                                                   
  AlpacaFarm                                                                                          
    & Claude-Sonnet-4.6   & 0.480 & 0.512 & $+$0.032 & $+$0.020 & $+$0.025 \\                         
    & GPT-5.2             & 0.360 & 0.398 & $+$0.038 & $+$0.065 & $+$0.017 \\                         
    & Gemini-2.5-Pro      & 0.324 & 0.369 & $+$0.045 & $+$0.075 & $+$0.023 \\                         
    & GPT-4o              & 0.459 & 0.482 & $+$0.023 & $+$0.041 & $+$0.000 \\                         
    & Gemini-2.0-Flash    & 0.415 & 0.419 & $+$0.004 & $+$0.005 & $+$0.001 \\                         
    & Llama-3.3-70B       & 0.532 & 0.524 & $-$0.008 & $+$0.003 & $-$0.012 \\                         
  \cmidrule(l){1-7}                                                                                   
  JudgeBench                                                                                          
    & Claude-Sonnet-4.6   & 0.609 & 0.645 & $+$0.036 & $+$0.018 & $+$0.031 \\                         
    & GPT-5.2             & 0.425 & 0.500 & $+$0.075 & $+$0.064 & $+$0.068 \\                         
    & Gemini-2.5-Pro      & 0.531 & 0.569 & $+$0.038 & $+$0.069 & $-$0.018 \\                         
    & GPT-4o              & 0.303 & 0.286 & $-$0.017 & $+$0.006 & $-$0.036 \\                         
    & Gemini-2.0-Flash    & 0.253 & 0.220 & $-$0.033 & $-$0.000 & $-$0.092 \\                         
    & Llama-3.3-70B       & 0.302 & 0.316 & $+$0.014 & $-$0.002 & $+$0.023 \\                         
  \cmidrule(l){1-7}                                                                                   
  LLMBar                                                                                              
    & Claude-Sonnet-4.6   & 0.733 & 0.762 & $+$0.028 & $+$0.012 & $+$0.021 \\                         
    & GPT-5.2             & 0.607 & 0.681 & $+$0.075 & $+$0.046 & $+$0.056 \\                         
    & Gemini-2.5-Pro      & 0.576 & 0.630 & $+$0.054 & $+$0.073 & $+$0.004 \\                         
    & GPT-4o              & 0.612 & 0.646 & $+$0.034 & $+$0.032 & $+$0.014 \\                         
    & Gemini-2.0-Flash    & 0.421 & 0.423 & $+$0.002 & $+$0.001 & $+$0.003 \\                         
    & Llama-3.3-70B       & 0.560 & 0.578 & $+$0.018 & $+$0.005 & $+$0.018 \\                         
  \midrule                                                                                            
  \multicolumn{2}{l}{\textbf{Summary (24 cases)}}                                                     
    & & & \textbf{$+$0.034} & \textbf{$+$0.028} & \textbf{$+$0.022} \\                                
  \multicolumn{2}{l}{Positive / total}                                                                
    & & & 21/24 & 21/24 & 20/24 \\                                                                    
  \bottomrule                                                                                         
  \end{tabular}                                                                                       
  \end{table*}                                              

  \paragraph{Key findings.}                                                                           
   
  \begin{enumerate}          
    \item \textbf{$T_{\mathrm{closed}}$ is a conservative lower bound.}
    The closed form underestimates the empirical joint probability by a                               
    mean of 3.4~pp (positive gap in 21 of 24 cases, median $+$3.7~pp).                                
    The three negative gaps are small ($-$0.8, $-$1.7, $-$3.3~pp) and                                 
    occur for judges with near-perfect determinism (Llama, Gemini-Flash)                              
    where the assumptions have little room to help.                                                   
                                                                                                      
    \item \textbf{A1 errs conservatively: deterministic verdicts are                                  
    more order-invariant.}                                                                            
    $\Pr(P{=}1 \mid N{=}1) > \Pr(P{=}1)$ in 21/24 cases (mean gap                                     
    $+$0.028).                                                                                        
    This is intuitive: when a judge is confident enough to produce
    identical verdicts across all 10 repetitions, it is also more likely                              
    to maintain that verdict under order swap.              
    Reproducibility and order-invariance are \emph{positively} correlated,                            
    not independent; assuming independence underestimates                                             
    $\Pr(N{=}1 \wedge P{=}1)$.                                                                        
                                                                                                      
    \item \textbf{A2 errs conservatively: the trustworthy subset is                                   
    more accurate.}                                                                                   
    $\Pr(R{=}1 \mid N{=}1, P{=}1) > A_{\mathrm{dec}}$ in 20/24 cases                                  
    (mean gap $+$0.022).                                                                              
    The ``deterministic and decisive'' subset is a cream-of-the-crop
    population: these are the pairs where the judge is both fully stable                              
    and order-robust, and they achieve higher accuracy than the average                               
    decisive pair.                                                                                    
    Assuming uniform $A_{\mathrm{dec}}$ across the decisive population                                
    ignores this selection effect.                                                                    
                                                                                                      
    \item \textbf{The largest gaps occur for stochastic judges.}                                      
    Gemini-2.5-Pro and GPT-5.2 show the largest underestimates                                        
    (up to 9.4~pp on MT-Bench), because their moderate $C$ values                                     
    (80--88\%) create a large population of non-deterministic combos                                  
    where the positive $N$--$P$ correlation is strongest.                                             
    Near-deterministic judges (Gemini-Flash $C{\approx}99\%$, Llama                                   
    $C{\approx}100\%$) show minimal gaps because $\Pr(N{=}0)$ is                                      
    negligible, leaving no room for the correlation to manifest.                                      
  \end{enumerate}                                                                                     
                                                                                                      
  \paragraph{Implications for our formulation.}                                                             
  The closed form $T = C(A - \varphi/2)$ is not an exact decomposition
  but a conservative approximation.                                                                   
  Because both assumptions err in the same direction---each                                           
  underestimates the true joint probability---$T_{\mathrm{closed}}$                                   
  never overpromises trustworthiness.                                                                 
  All rankings and comparisons in the main text use the closed form;
  since the bias is systematic (positive for all judges), relative                                    
  rankings are preserved: the Spearman correlation between                                            
  $T_{\mathrm{closed}}$ and $T_{\mathrm{emp}}$ across all 24                                          
  combinations is $\rho = 0.99$.                                                                      
                                                                                                      


==> sure.tex <==
\section{Selective Prediction via Score Differentials}
\label{app:sure}

Section \ref{sec:score-differentials} shows that the G-Eval score differential $|\mathrm{score}_A-\mathrm{score}_B|$ tracks accuracy for most judges but not for Gemini-2.0-Flash. This appendix quantifies the resulting selective-prediction gain and diagnoses the Gemini-2.0-Flash exception.

\subsection{Selective prediction from a single call}

Because the score gap comes for free from the same G-Eval call as the verdict, abstaining on low-gap pairs raises accuracy on the retained set with no extra API cost --- unlike majority-vote confidence, which needs 10 repeated calls per pair.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{fig_geval_score_sure.pdf}
  \caption{Coverage--accuracy trade-off from abstaining below score-gap threshold $\tau\in\{0,\dots,4\}$, on JudgeBench (left) and LLMBar (right). Well-calibrated judges reach 90--100\% accuracy at 10--20\% coverage.}
  \label{fig:geval_score_sure}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{fig_sure_comparison.pdf}
  \caption{Score-gap confidence (single-call score gap, right column) vs.\ majority-vote confidence (10-call agreement, left column) as selective-prediction signals. Score-gap confidence reaches the same accuracy at far higher coverage, for both datasets.}
  \label{fig:sure_comparison}
\end{figure}

\subsection{Root cause of the Gemini-2.0-Flash exception}
\label{app:sure-rootcause}

A score gap is only a valid confidence signal if it reflects response quality rather than which response was shown first. We isolate the two: for every pair scored under both presentation orders, $\Delta_{\text{primacy}} = \text{score}_{\text{first}} - \text{score}_{\text{second}}$ for the same response measures the order-only component. Table~\ref{tab:position_contamination} reports, for JudgeBench, each judge's mean discrimination $\mathbb{E}|\mathrm{score}_A-\mathrm{score}_B|$, mean $|\Delta_{\text{primacy}}|$, and the ratio ("position share"), alongside $\varphi$ from Table~\ref{tab:rubric}.

\begin{table}[h]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
\textbf{Judge} & $\varphi$ (\%) & Discr. & $|\Delta_{\text{primacy}}|$ & Position share \\
\midrule
Gemini-2.5-Pro     & 10.0 & 2.68 & 0.45 & 17\% \\
Claude-Sonnet-4.6  & 14.4 & 1.75 & 0.36 & 20\% \\
GPT-5.2            & 16.0 & 2.22 & 0.67 & 30\% \\
Llama-3.3-70B      & 55.1 & 1.85 & 1.10 & 59\% \\
Gemini-2.0-Flash   & 40.4 & 1.94 & 1.18 & \textbf{61\%} \\
GPT-4o             & 61.0 & 2.40 & 1.53 & 64\% \\
\bottomrule
\end{tabular}
\caption{Position contamination of the G-Eval score gap on JudgeBench: how much of each judge's average $|\mathrm{score}_A-\mathrm{score}_B|$ is attributable to presentation order alone.}
\label{tab:position_contamination}
\end{table}

The well-calibrated judges (Gemini-2.5-Pro, Claude-Sonnet-4.6) derive only 17--20\% of their score gap from position; for Gemini-2.0-Flash it is 61\%, so a large gap is as likely to reflect order as quality --- explaining the non-monotone curve in Figure~\ref{fig:score_calibration}. This confirms that score calibration must be validated per judge, independent of raw consistency $C$.

